Selective Memoization

This paper presents language techniques for applying memoization selectively. The techniques provide programmer control over equality, space usage, and identification of precise dependences so that memoization can be applied according to the needs of an application. Two key properties of the approach are that it accepts and efficient implementation and yields programs whose performance can be analyzed using standard analysis techniques. We describe our approach in the context of a functional language called MFL and an implementation as a Standard ML library. The MFL language employs a modal type system to enable the programmer to express programs that reveal their true data dependences when executed. We prove that the MFL language is sound by showing that that MFL programs yield the same result as they would with respect to a standard, non-memoizing semantics. The SML implementation cannot support the modal type system of MFL statically but instead employs run-time checks to ensure correct usage of primitives.

==> adaptivity.tex <==
\section{Memoization and Adaptivity} 
\label{sec:adaptivity}
This work was motivated by our previous work on adaptive
computation~\cite{AcarBlHa02}.  In this section, we briefly discuss the
relationship between memoization and adaptivity and how they can be
combined to obtain efficient dynamic or incremental algorithms.

An adaptive computation maintains a dynamic dependence graph representing
data and control dependences.  When the input is modified, a change
propagation algorithm updates the output and the dependence graph.  The
adaptivity mechanism handles ``deep'' changes efficiently.  We say that a
change is {\em deep} if it affects calls that occur at leaves of the call
tree for the computation. In contrast, a change is {\em shallow} if it
affects by a calls that occur at the roots of the call three.

As an example consider the Quicksort algorithm that picks the first key of
its input as pivot. Inserting a new key at the end of the input list is a
deep change because this change will affect the last recursive calls of
some filter functions and will become pivot only at the end of some
sequence of recursive calls to Quicksort.  In contrast, inserting a new
key at the beginning of the list is a shallow change for Quicksort,
because the new key will be selected as a pivot immediately by the first
call to the Quicksort.  The adaptivity mechanism based on dynamic
dependence graphs handles an insertion at the end of the input, a deep
change, in expected $O(\log{n})$ time, whereas the insertion at the
beginning of the list, a shallow change, will cause a complete rerun,
which takes $O(n\log{n})$ time.  Using memoization, however, an insertion
at the beginning of the list can be handled in $O(n)$ time as we show in
\secref{framework}.  

Any change can be thought of a combination of shallow and deep changes.
Since memoization and adaptivity complement each other in their handling
of deep and shallow changes, we would expect that a combination of these
two techniques would handle general changes efficiently.  For example, in
Quicksort, we expect that an insertion in a random position in the list
would be handled in expected $O(\log{n})$ time by a combination of these
two techniques.

Combining the adaptivity with the memoization framework desribed here is
relatively straightforward but requires some changes to both libraries.
In fact, we have an initial implementation that combines these two
techniques.  Our experience so far indicates that more sophisticated
memoization techniques are required to realize sophisticated dynamic
algorithms.  These memoization techniques would allow the programmer to
re-use a ``partial'' (\ie, not correct) result and ``fix'' the result via
adaptivity.




==> box-fig.tex <==
\begin{figure}
\centering{\fbox{
\parbox[t]{4in}{
\begin{codeListingS}
XX\=\kill

signature BOX = \\
sig\\
\>type 'a box\\[2mm]
\>val init:unit -> unit\\
\>val box:'a -> 'a box\\
\>val unbox:'a box -> 'a\\
\>val keyOf:'a box -> int\\
end
\end{codeListingS}}}}
\caption{The signatures for boxes.}
\label{fig:box}
\end{figure}

==> box-memo-fig.tex <==
\begin{figure}
\centering{\fbox{
\parbox[t]{1.5in}{
\begin{codeListingS}
signature BOX = \\
sig\\
\>type 'a box\\
\>val init:unit -> unit\\
\>val box:'a -> 'a box\\
\>val unbox:'a box -> 'a\\
\>val keyOf:'a box -> int\\
end

\end{codeListingS}}}}
\caption{The signatures for boxes.}
\label{fig:sig}
\end{figure}

==> memo-fig.tex <==
\begin{figure}
\centering{\fbox{
\parbox[t]{1.5in}{
\begin{codeListingS}
signature MEMO_TABLE = \\
sig\\
\>type 'a memotable\\
\>type index\\[2mm]

\>val empty: unit -> 'a memotable\\
\>val extend: 'a memotable -> index list -> ('a option * 'a memotable option)\\
\> val add: 'a -> 'a memotable -> unit\\
end
\end{codeListingS}}}}
\caption{The signatures for memo tables.}
\label{fig:box}
\end{figure}

==> reviews.tex <==
============================================================================ 
POPL03 Reviews for Paper #133
============================================================================ 

Title: Selective Memoization

Authors: Umut A. Acar and Guy E. Blelloch and Robert Harper

============================================================================ 

REVIEWER #1
============================================================================ 

Numerical Scores:

     appropriateness: 5
     originality: 4
     tech_strength: 4
     presentation: 2
     overall: 4


Comments:

The use of memo-functions is an attractive feature of
programming. However, an uncontroled use leads to explosion in memory
space and to unefficiency. This paper studies selected memoization,
i.e. a mini-language for specifying functional programs with support
for cache handling and memoization selected by the programmer.

In this language, there are two categories of programming
constructs. The first ones are terms which are non-memoized and
evaluate to standard (functional) values. A memoized function value
also returns a new cache table if not already existing (There are as
many cache tables as many functions). The second category forms the
set of expressions which are the memoized following constructs:
"return", "let!", "letX" and "mcase".  The "mcase" switches on a sum
type with two variants and keeps the trace of the choice. The "let!"
is a standard let construct, which keeps the value computed for the
bound variable. The "letX" is a standard destructor on pairs. The
"result" statement looks at the trace of registered values and choices
needed to access to that statement and searches for a cache entry of
the current function with the current trace. If one does exist, the
term is not evaluated and "return" provides its value; if none, the
term evaluation is performed and a cache entry is!  created for this
pair: trace and value.

Thus the good usage of "let!", "mcase" and "return" statements gives a
flexibility in the level of memoization for results, as explained in
the first example for the Fibonacci function. Also the caching of
control in "mcase" makes it possible for partial cache (illustrated in
the second example with a binary sum), since the only possible
information is the control and not the value of the arguments.

The static and dynamic semantics of the language is given, in a short
and succinct way (which does not seem obvious for me). A soundness
theorem is provided at the end of the paper, ensuring that the
computed values with memoization are sound, wrt non-memoized
language. The proof is in the appendix and seems trustable.

The extra cost involved by cache lookups is no more than a constant
factor, since the cache lines stores the control. But the speedup may
be as high as the length of computation of a cached value. An
implementation has been achieved in SML, and the authors notice its
simplicity.

The paper is not so well written, and looks to have been produced in a
rush. There are several typos (some are mentioned at end of this
report). The technical explanation is short, whereas the introduction
+ overview is quite long. The work also seems an extension of the
adaptive language (POPL'02 by same authors). But my understanding of
the POPL'02 paper is that it's more on incremental computations than
on caching. The paper also differs from fine grained dependency
analysis (as Abadi et al, Heydon et al), and provides an easier
implementation (but with loosing elegancy).

An important unresolved problem is still memory-space explosion, since
there is no reclaim of cache tables or cache lines (never the sigma's
or the beta's vanished in the tables of fig. 7-8). It is also noticed
by the authors in the conclusion, which makes invalid one of the
initial claims. Tables may vanished with scope of function which seems
a minimal requirement. But fixing this memory leak is not obvious.

Altogether, the authors demonstrate their good knowledge of the
memoization problem. The techniques seem correct. There is an
implementation. The paper shows some interest for situating the
memoization problem.

Typos or short remarks:

p.6 line 2: when $n_1$ is NOT positive

p.6 line -6: more likely to return the same result THAN some other function

p.8 fig 4: Do we really need "x" in values?

p.11 in def of memo table the empty set is missing, but used in fig 7

p.12: fig 7: (Apply) [v1/f, v2/a] is more consistent with fig 8.

p.12: fig 7: (Roll) (Unroll) are never explained!

============================================================================
REVIEWER #2
============================================================================ 

Numerical Scores:

     appropriateness: 5
     originality: 4
     tech_strength: 3
     presentation: 4
     overall: 4


Comments:

 Summary
-------

This paper describes an extended version of ML which accommodates
memoization of function results.  The new language features allow a
programmer to specify what parts of a function's arguments "tracked"
at runtime; those parts of the arguments that are actually inspected
by the function are then used to allow memoized results to be reused
on functions whose arguments are not identical, but whose result
depends on identical _parts_ of the arguments.  It also allows the
programmer to selectively specify which data constructors are
hash-consed, to allow fast equality testing for retrieving memoized
values.  By allowing programmers to use memoization selectively, its
cost (which can sometimes exceed its value) can be understood and
controlled.  The ML type system is extended in a way that ensures that
dependence tracking information is used consistently.  The paper
supplies the details of the "modal" type system used to track
dependencies, an operational semantics of memoized function
application, some details on an implementation of the approach using a
library written in unadorned ML, and a proof of correspondence between
the memoized and non-memoized versions of the code.

Points in Favor/Against
-----------------------

+ Nice combinations of features for adding memoization to an
  existing functional language in a controlled way

+ Useful extension of the ML type system to ensure consistent
  annotation

+ Notion of keying memo tables on a program path was interesting
  and novel to this reviewer

+ Generally clearly-written (aside from typos)

- Not clear how easy it is to annotate large programs effectively

- No empirical results


General Evaluation
------------------

I liked this paper a lot.  While none of the ingredients of the
approach are particularly deep, taken together, they provide a nice
balance between giving the programmer adequate control over resource
management and ensuring safety and correctness.  The interplay between
types and an optimized execution strategy is very pleasant.  The
notion of keying memo tables on a control-flow path was novel to me,
and seems to be the linchpin of the whole approach.  This is the first
language extension I have seen that supports memoization and
hash-consing in a way that provides enough control for programmers to
consider actually using it.

Major Comments
--------------

- It would be nice to provide a compelling example where the modal
  operations aren't "obvious" from the contents of a return
  expression.

- You state on p.5 that mcase "records the branch taken" (and use,
  e.g., mcase with boolean expressions later on), but the formal
  semantics only considers branches derived from matches against "inl"
  and "inr".

- p.4, para.1: I don't completely understand how a fine-grained
  labeling policy can change the time complexity of a function (is the
  issue that the generation of labels can take longer than the
  computation itself)?  Some elaboration here would be useful,
  especially since the topic comes up again when you discuss "deep"
  dependencies later on.  Also, you criticize a labeling policy based
  on a "meta-language"< but your "necessitation" modality amounts to a
  kind of meta-language as well.

- p.5: You never really explain the "!" operator for values.  This
  is compounded by the fact that it seems to be used inconsistently
  later on.  For example, "hash-cons" in Fig. 2 returns a value
  without "!", whereas "msearch" returns a value with "!".

- p.6, para.1: "This sort of examples are [example is?] easily
  expressed in our framework": While I think I know what you have in
  mind, an example of this sort of thing would be nice.  In fact, your
  ability to accommodate cases such as this seems to be a significant
  advantage of your method.

- p.8, para.1: "the techniques for adding such a mechanism are
  well-understood".  Maybe, but if so, you should provide a reference.

- Section 4.2: The discussion of the origins of the modal type system
  may be interesting to specialists, but distracts from the
  presentation of the main ideas.  E.g., I was left wondering exactly
  what a "monadic interpretation of memoization" might be (should I
  care?)

- Fig.5: What are "roll" and "unroll" used for?

- p.11, footnote 4: I don't understand this comment.  Don't memo
  tables always "respect value equivalence"?

- Section 4.5: The really interesting performance issue is how much
  performance degradation the "constant" time overhead really entails
  (as well as how much speedup memoization in general allows).  After
  all, hash-consing and memoizing absolutely everything also has only
  "constant-time" overhead.

- Section 5: This is pretty hard to follow without more details about
  the implementation (which I guess you were forced to relegate to the
  appendix...).  For example, I don't understand the last sentence in
  para.2 on p. 15.

- Even though a memoized function is asymptotically no slower than a
  non-memoized function, there is clearly a non-negligible constant
  factor overhead.  What is it?  The paper described an implementation
  but no empirical results.

- Do you have any thoughts on how imperative aspects of ML could
  be handled by your technique?

Minor Comments
--------------

- Fig.2, non-memoized "compare", should (I assume) not have "!" in argument

- Fig.3, "case" in memoized version should (I assume) be "mcase"

- p.6, line 3: "not" -> "does not"

- p.6, line -6: "then" -> "than"

- p.7, line -1: "efficenent" -> "efficient

============================================================================
REVIEWER #3
============================================================================ 

Numerical Scores:

     appropriateness: 5
     originality: 4
     tech_strength: 4
     presentation: 5
     overall: 4


Comments:

 The paper sets up a framework in which programmers can express the
details of memoization. The first idea is to introduce a notion of
resources which have special types and restricted access: a memoized
function accesses the resources using any of the available primitives
on resources and then returns a value. The value is then automatically
associated with this sequence of resource operations on any future
call. Also essential (but less innovative in some sense) are
constructs giving programmers control over how equality is
implemented, and over the scope of memo tables. Technically the paper
introduces a small functional language with the necessary primitives
and a modal type system and establishes soundness of memoized
evaluation with respect to pure evaluation, and hence type
soundness. It also describes an implementation of the basic idea
(without the modal type system) in an SML library.

The paper is very well-written and enjoyable to read.

============================================================================

==> soundness.tex <==
\section{Soundness}
\label{app:mfl-sound}
\label{app:soundness}

We will prove the soundness of \MFL{} relative to a non-memoizing semantics for
the language.  It is straightforward to give a purely functional semantics to
\MFL{} by an inductive definition of the relations $\t\treducespure \v$ and
$\e\ereducespure\v$, where $\v$ is a \emph{pure value} with no location
subscripts (see, for example,~\cite{pfenning+:judgmental}).  We will show that,
under suitable conditions, memoization does not affect the outcome of
evaluation as compared to the non-memoized semantics.  To make this precise, we
must introduce some additional machinery.

The \emph{underlying term}, $\ers{\t}$, of a term, $\t$, is obtained by erasing
all location subscripts on function values occurring within $\t$.  The
\emph{underlying expression}, $\ers{\e}$, of an expression, $\e$, is defined in
the same way.  As a special case, the \emph{underlying value}, $\ers{\v}$, of a
value, $\v$, is the underlying term of $\v$ regarded as a term.  It is easy to
check that every pure value arises as the underlying value of some impure
value.  Note that passage to the underlying term or expression obviously
commutes with substitution.  The \emph{underlying branch}, $\ers{\beta}$, of a
simple branch, $\beta$, is obtained by replacing each event of the form
$\bang{\v}$ in $\beta$ by the corresponding underlying event,
$\bang{(\ers{\v})}$.

\smallskip

The partial \emph{access functions}, $\atbr{\t}{\br}$ and $\atbr{\e}{\br}$,
where $\br$ is a simple branch, and $\t$ and $e$ are variable-free (but not
necessarily resource-free), are defined as follows.  The definition may be
justified by lexicographic induction on the structure of the branch followed by
the size of the expression.
\begin{displaymath}
  \begin{array}{rcl}
    \atbr{\t}{\br} & = & \atbr{\e}{\br}
    \\
    \multicolumn{3}{r}{
      (\textit{where}\ \t=\fun{f}{a}{\taui}{\tauii}{\e})
    }
    \\ \\
    \atbr{\ret{\t}}{\nullbr} & = & \ret{\t} \\
    \atbr{\letbin{x\cdcolon\tau}{\t}{\e}}{\bangbr{\br}{\v}} & = & \atbr{\subst{v}{x}{\e}}{\br} \\
    \atbr{\letpin{a_1\cdcolon\taui}{a_2\cdcolon\tauii}{\t}{\e}}{\br} & = &
    \atbr{\e}{\br} \\
    \atbr{\caseofflat{\t}{a_1}{\taui}{\e_1}{a_2}{\tauii}{\e_2}}{\inlbr{\br}} &
    = & \atbr{\e_1}{\br} \\
    \atbr{\caseofflat{\t}{a_1}{\taui}{\e_1}{a_2}{\tauii}{\e_2}}{\inrbr{\br}} &
    = & \atbr{\e_2}{\br} \\
  \end{array}
\end{displaymath}
This function will only be of interest in the case that $\atbr{\e}{\br}$ is a
\textcd{return} expression, which, if well-typed, cannot contain free
resources.  Note that $\ers{(\atbr{\e}{\br})} = \atbr{\ers{\e}}{\ers{\br}}$,
and similarly for values, $\v$.

We are now in a position to justify a subtlety in the second \textcd{return}
rule of the dynamic semantics, which governs the case that the returned value
has not already been stored in the memo table.  This rule extends, rather than
updates, the memo table with a binding for the branch that determines this
\textcd{return} statement within the current memoized function.  But why, after
evaluation of $\t$, is this branch undefined in the revised store, $\msp$?  If
the term $\t$ were to introduce a binding for $\br$ in the memo table
$\sigma(l)$, it could only do so by evaluating the very same \textcd{return}
statement, which implies that there is an infinite loop, contradicting the
assumption that the \textcd{return} statement has a value, $\v$.
\begin{lemma}
\label{lemma:at-undef}
  If $\tis{\ms}{\t}\treduces\tos{v}{\msp}$, $\atbr{\sigma(l)}{\br}=\ret{\t}$,
  and $\ms(l)(\br)$ is undefined, then $\msp(l)(\br)$ is also undefined.
\end{lemma}

\smallskip

An \emph{augmented branch}, $\gbr$, is an extension of the notion of branch in
which we record the bindings of resource variables.  Specifically, the argument
used to call a memoized function is recorded, as are the bindings of resources
created by pair splitting and case analysis.  Augmented branches are
inductively defined by the following grammar:
\begin{displaymath}
  \begin{array}{lrcl}
    \textit{Augmented Event} & \gev & \bnfdef & \callgev{\v} \bnfalt
    \banggev{\v} \bnfalt \pairgev{\vi}{\vii} \bnfalt \inlgev{\v} \bnfalt
    \inrgev{\v} \\ 
    \textit{Augmented Branch} & \gbr & \bnfdef & \nullgbr \bnfalt
    \consgbr{\gev}{\gbr} \\
  \end{array}
\end{displaymath}
We write $\extgbr{\gbr}{\gev}$ for the extension of $\gbr$ with $\gev$ at the
end.  There is an obvious \emph{simplification} function, $\simp{\gbr}$, that
yields the simple branch corresponding to an augmented branch by dropping
``call'' events, $\callgev{\v}$, and ``pair'' events, $\pairgev{\vi}{\vii}$,
and by omitting the arguments to ``injection'' events, $\inlgev{\v}$,
$\inrgev{\v}$.  The \emph{underlying augmented branch}, $\ers{\gbr}$,
corresponding to an augmented branch, $\gbr$, is defined by replacing each
augmented event, $\gev$, by its corresponding underlying augmented event,
$\ers{\gev}$, which is defined in the obvious manner.  Note that
$\ers{(\simp{\gbr})} = \simp{(\ers{\gbr})}$.

The partial access functions $\atgbr{\e}{\gbr}$ and $\atgbr{\t}{\gbr}$ are
defined for closed expressions $e$ and closed terms $t$ by the following
equations:
\begin{displaymath}
  \begin{array}{rcl}
    \atgbr{\t}{\callgbr{\gbr}{\v}} & = & \atgbr{\subst{\t,\v}{f,a}{\e}}{\gbr}
    \\
    \multicolumn{3}{r}{
      (\textit{where}\ \t=\fun{f}{a}{\taui}{\tauii}{\e})
    }
    \\ \\
    \atgbr{\e}{\nullgbr} & = & e \\
    \atgbr{\letbin{x\cdcolon\tau}{\t}{\e}}{\banggbr{\gbr}{\v}} & = &
    \atgbr{\subst{\v}{x}{\e}}{\gbr} \\
    \atgbr{\letpin{a_1\cdcolon\taui}{a_2\cdcolon\tauii}{\t}{\e}}{\splitgbr{\br}{\vi}{\vii}} & = & \atgbr{\subst{\vi,\vii}{a_1,a_2}{\e}}{\br} \\
    \atgbr{\caseofflat{\t}{a_1}{\taui}{\e_1}{a_2}{\tauii}{\e_2}}{\inlgbr{\br}{\v}} & = & \atgbr{\subst{\v}{a_1}{\e_1}}{\br} \\
    \atgbr{\caseofflat{\t}{a_1}{\taui}{\e_1}{a_2}{\tauii}{\e_2}}{\inrgbr{\br}{\v}} & = & \atgbr{\subst{\v}{a_2}{\e_2}}{\br} \\
  \end{array}
\end{displaymath}
Note that $\ers{(\atgbr{\e}{\gbr})} = \atgbr{\ers{\e}}{\ers{\gbr}}$, and
similarly for values, $\v$.

Augmented branches, and the associated access function, are needed for the
proof of soundness.  The proof maintains an augmented branch that enriches the
current simple branch of the dynamic semantics.  The additional information
provided by augmented branches is required for the induction, but it does not
affect any \textcd{return} statement it may determine.
\begin{lemma}
\label{lemma:at-simp}
  If $\atgbr{\e}{\gbr}=\ret{\t}$, then $\atbr{\e}{\simp{\gbr}}=\ret{\t}$.
\end{lemma}

A \emph{function assignment}, $\MS$, is a finite mapping from locations to
well-formed, closed, pure function values.  A function assignment is
\emph{consistent with} a term, $t$, or expression, $e$, if and only if whenever
$\funval{l}{f}{a}{\taui}{\tauii}{e}$ occurs in either $t$ or $e$, then
$\MS(l)=\fun{f}{a}{\taui}{\tauii}{\ers{e}}$.  Note that if a term or expression
is consistent with a function assignment, then no two function values with
distinct underlying values may have the same label.  A function assignment is
consistent with a store, $\ms$, if and only if whenever $\ms(l)(\br)=\v$, then $\MS$ is
consistent with $\v$.

A store, $\ms$, \emph{tracks} a function assignment, $\MS$, if and only if $\MS$ is
consistent with $\sigma$, $\dom{\ms}=\dom{\MS}$, and for every $l\in\dom{\ms}$,
if $\ms(l)(\br)=\v$, then
\begin{enumerate}
\item $\atbr{\MS(l)}{\ers{\br}}=\ret{\ers{\t}}$,
\item $\ers{\t}\treducespure\ers{\v}$,
\end{enumerate}
Thus if a branch is assigned a value by the memo table associated with a
function, it can only do so if that branch determines a \textcd{return}
statement whose value is the assigned value of that branch, relative to the
non-memoizing semantics.

We are now in a position to prove the soundness of \MFL{}.
\begin{thm}
  \begin{enumerate}
  \item If $\tis{\ms}{\t}\treduces\tos{\v}{\msp}$, $\MS$ is consistent with
    $\t$, $\ms$ tracks $\MS$, $\emptyContext;\emptyContext\ts \t:\tau$, then
    $\ers{\t}\treducespure \ers{\v}$ and there exists $\MSP\supseteq\MS$ such
    that $\MSP$ is consistent with $\v$ and $\msp$ tracks $\MSP$.
  \item If $\eis{\ms}{l}{\br}{\e}\ereduces\eos{\v}{\msp}$, $\MS$ is consistent
    with $e$, $\ms$ tracks $\MS$, $\simp{\gbr}=\br$,
    $\atgbr{\MS(l)}{\ers{\gbr}}=\ers{\e}$, and $\emptyContext;\emptyContext\ts
    \e:\tau$, then there exists $\MSP\supseteq\MS$ such that
    $\ers{\e}\ereducespure\ers{\v}$, $\MSP$ is consistent with $\v$, and $\msp$
    tracks $\MSP$.
  \end{enumerate}
\end{thm}
\begin{proof}
  The proof proceeds by simultaneous induction on the memoized evaluation
  relation.  We consider here the five most important cases of the proof:
  function values, function terms, function application terms, and return
  expressions.
  
  For function values $\t=\funval{l}{f}{a}{\taui}{\tauii}{\e}$, simply take
  $\MSP=\MS$ and note that $\v=\t$ and $\msp=\ms$.
  
  For function terms $\t=\fun{f}{a}{\taui}{\tauii}{\e}$, note that
  $\v=\funval{l}{f}{a}{\taui}{\tauii}{\e}$ and $\msp=\ms[l\mapsto\emptyset]$,
  where $l\notin\dom{\ms}$.  Let $\MSP=\MS[l\mapsto \ers{\v}]$, and note that
  since $\ms$ tracks $\MS$, and $\ms(l)=\emptyset$, it follows that $\msp$
  tracks $\MSP$.  Since $\MS$ is consistent with $\t$, it follows by
  construction that $\MSP$ is consistent with $\v$.  Finally, since
  $\ers{\v}=\ers{\t}$, we have $\ers{\t}\treducespure\ers{\v}$, as required.
  
  For application terms $\t=\apply{\ti}{\tii}$, we have by induction that
  $\ers{\ti}\treducespure\ers{\vi}$ and there exists $\MSi\supseteq\MS$
  consistent with $\vi$ such that $\msi$ tracks $\MSi$.  Since
  $\vi=\funval{l}{f}{a}{\taui}{\tauii}{\e}$, it follows from consistency that
  $\MSi(l)=\ers{\vi}$.  Applying induction again, we obtain that
  $\ers{\tii}\treducespure\ers{\vii}$, and there exists $\MSii\supseteq\MSi$
  consistent with $\vii$ such that $\msii$ tracks $\MSii$.  It follows that
  $\MSii$ is consistent with $\subst{\vi,\vii}{f,a}{\e}$.  Let
  $\gbr=\consgbr{\callgev{\vii}}{\nullgbr}$.  Note that
  $\simp{\gbr}=\nullbr=\br$ and we have
  \begin{displaymath}
    \begin{array}{rcl}
      \atgbr{\MSii(l)}{\ers{\gbr}} & = & \atgbr{\ers{\vi}}{\ers{\gbr}} \\
      & = & \ers{(\atgbr{\vi}{\gbr})} \\
      & = & \ers{(\subst{\vi,\vii}{f,a}{\e})} \\
      & = & \subst{\ers{\vi},\ers{\vii}}{f,a}{\ers{\e}}.
    \end{array}
  \end{displaymath}
  Therefore, by induction,
  $\subst{\ers{\vi},\ers{\vii}}{f,a}{\ers{\e}}\ereducespure\ers{\vp}$, and
  there exists $\MSP\supseteq\MSii$ consistent with $\vp$ such that $\msp$
  tracks $\MSP$.  It follows that $\ers{(\apply{\ti}{\tii})} =
  \apply{\ers{\ti}}{\ers{\tii}}\treducespure\ers{\vp}$, as required.
  
  For return statements, we have two cases to consider, according to whether
  the current branch is in the domain of the current memo table.  Suppose that
  $\eis{\ms}{l}{\br}{\ret{\t}}\ereduces\eos{\v}{\msp}$ with $\MS$ consistent
  with $\ret{\t}$, $\ms$ tracking $\MS$, $\simp{\gbr}=\br$,
  $\atgbr{\MS(l)}{\ers{\gbr}}=\ers{(\ret{\t})}=\ret{\ers{\t}}$, and
  $\emptyContext;\emptyContext\ts \ret{\t}:\tau$.  Note that by
  Lemma~\ref{lemma:at-simp}, $\ers{(\atbr{\MS(l)}{\br})} =
  \atbr{\MS(l)}{\ers{\br}} = \ret{\ers{\t}}$.
  
  For the first case, suppose that $\ms(l)(\br)=\v$.  Since $\ms$ tracks $\MS$
  and $l\in\dom{\ms}$, we have $\MS(l)=\fun{f}{a}{\taui}{\tauii}{\ers{\e}}$
  with $\atbr{\ers{\e}}{\ers{\br}}=\ret{\ers{\t}}$, and
  $\ers{\t}\treducespure\ers{\v}$.  Note that $\msp=\ms$, so taking $\MSP=\MS$
  completes the proof.
  
  For the second case, suppose that $\ms(l)(\br)$ is undefined.  By induction
  $\ers{\t}\treducespure\ers{\v}$ and there exists $\MSP\supseteq\MS$
  consistent with $\v$ such that $\msp$ tracks $\MSP$.  Let $\theta'=\msp(l)$,
  and note $\theta'(\br)\uparrow$, by Lemma~\ref{lemma:at-undef}.  Let
  $\theta''=\theta'[\br\mapsto\v]$, and $\mspp=\msp[l\leftarrow\theta'']$.  Let
  $\MSPP=\MSP$; we are to show that $\MSPP$ is consistent with $\v$, and
  $\mspp$ tracks $\MSPP$.  By the choice of $\MSPP$ it is enough to show that
  $\atbr{\MSP(l)}{\ers{\br}}=\ret{\ers{\t}}$, which we noted above.
  
\end{proof}

Type safety follows from the soundness theorem, since type safety holds for the
non-memoized semantics.  In particular, if a term or expression had a
non-canonical value in the memoized semantics, then the same term or expression
would have a non-canonical value in the non-memoized semantics, contradicting
safety for the non-memoized semantics.

%Type safety, which states the coherence of the static and dynamic semantics,
%may be proved for \MFL{} using standard
%techniques~\cite{wrightfelleisen,harper-refs}.  Since we are working with an
%evaluation semantics, the argument is indirect.  First, we prove type
%preservation, which states that the value of a term or expression has the same
%type as the expression.  Since our semantic values are not forms of expression,
%this requires that we explicitly define a typing relation for semantic values.
%Second, we characterize the canonical values of each type.  Using this we may
%then prove safety by instrumenting the dynamic semantics to ``go wrong''
%whenever the value of a principal argument of an elimination form is not
%canonical.

%\begin{thm}
%  \begin{enumerate}
%  \item If $\tis{\ms}{\t}\treduces\tos{\v}{\msp}$, with $\ms:\MS:\Gamma$
%    and $\Gamma;\emptyContext\ts \t:\tau$, then $\Gamma\ts\v:\tau$.
%  \item If $\eis{\ms}{l}{\br}{\e}\ereduces\eos{\v}{\msp}$, with
%    $\ms:\MS:\Gamma$ and $\Gamma;\emptyContext\ts \e:\tau$, then
%    $\Gamma\ts v:\tau$.
%  \end{enumerate}
%\end{thm}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 








==> typing-figure.tex <==
%% typing  for external values
\begin{figure}[h]
\fixedCodeFrame{
\small
\setlength{\tabcolsep}{0ex}
\[
\begin{array}{c}
% Variables, Resources
\infer[\rlabel{variable}]  {\G ; \D  \ts x \cc \tau} {(\G(x)=\tau)}
\quad\quad
% Resources
\infer[\rlabel{resource}]  {\G ; \D  \ts a \cc \tau} {(\D(a)=\tau)}
\\[4mm]

% Constants
\infer[\rlabel{number}]  {\G ; \D  \tsi n : \Int}{\strut} 
\quad\quad
\infer[\rlabel{unit}]  {\G ; \D  \tsi \uno : \tunit}{\strut} 
\\[4mm]

% Primitives
\infer [\rlabel{primitive}]
{\G ; \D  \ts \op{\ti,\ldots,\t_n} : \tau}
{\G ; \D  \ts \t_i : \tau_i ~~(1\leq i\leq n) ~&~ \tso \oper
:(\taui, \ldots, \tau_n)~\tau}
\\[4mm]

\infer[\rlabel{pair}]
{\G ; \D \ts \pair{\ti}{\tii} :\taui \cross \tauii}
{\G ; \D  \ts \ti : \taui & 
\G ; \D  \ts \tii : \tauii}
\\[4mm]

%{First and Second}
%&
%\raisebox{-2ex}{\mbox{$
%\infer  {\G ; \D \ts \first{\t} :\taui}
%        {\G ; \D  \ts \t : \taui \cross \tauii}
%\quad\quad
%\infer  {\G ; \D \ts \second{\t} :\tauii}
%        {\G ; \D  \ts \t : \taui \cross \tauii}
%$}} \tablerow{}


%% Fun
\infer[\rlabel{fun}]
{\G ; \D  \tsi \fun{f}{a}{\taui}{\tauii}{\e}  : \taui \ra \tauii}
{\G ,\, f \cc \taui \ra \tauii;\D,a\cc \taui \ts \e :\tauii}
\\[4mm]

%%Fun val
\infer[\rlabel{fun value}]
{\G; \D \tsi \funval{l}{f}{a}{\taui}{\tauii}{\e} : \taui\ra\tauii}
{\G,f\cc\taui\ra\tauii; \D,a\cc\taui \ts \e:\tauii}
\\[4mm]

% Apply
\infer [\rlabel{apply}]
{\G ; \D  \ts \apply{\ti}{\tii} : \tauii}
{\G ; \D \ts \ti: \taui \ra \tauii & \G ;  \D  \ts \tii : \taui}
\\[4mm]

%Bang 
\infer[\rlabel{bang}]
{\G ; \D  \ts \bang{\t} : \bang{\eta}}
{\G ; \emptyContext  \ts \t : \eta}
\\[4mm]

%Sum
\infer[\rlabel{sum/inl}]
{\G ; \D  \ts \inl{\t}{\taui}{\tauii} : \taui \osum \tauii}
{\G ; \D  \ts \t : \taui} \qquad
\infer[\rlabel{sum/inr}]
{\G ; \D  \ts \inr{\t}{\taui}{\tauii} : \taui \osum \tauii}
{\G ; \D  \ts \t : \tauii}
\\[4mm]

%{Roll, Unroll}
\infer[\rlabel{roll}]
{\G ; \D  \ts \roll{\t} : \rt{\u}{\tau} }
{\G ; \D  \ts \t : [\rt{\u}{\tau}/\u]\tau}
\qquad
\infer[\rlabel{unroll}]
{\D  \ts \unroll{\t} :  [\rt{\u}{\tau}/\u]\tau}
{\G ; \D  \ts \t :\rt{\u}{\tau}}
% {Case}
% &
% \raisebox{-2ex}{\mbox{$
% \infer  {\G ; \D \ts \caseofflat{\t}{\ai}{\taui}{\ti}{\aii}{\tauii}{\tii} : \tau}
%         {
%         \begin{array}{rcl}
%         \G ; \D & \ts &  t : \taui \osum \tauii \\
%         \G; \D,\ai\cc\taui & \ts & \ti : \tau\\
%         \G; \D,\aii\cc\tauii & \ts & \tii : \tau
%         \end{array}
% }
% $}} \tablerow{}



%{Box and Unbox}
%&
%\raisebox{-2ex}{\mbox{$
%\infer  {\G ; \D  \ts \mbx{\t} : \bxed{\tau} }
%        {\G ; \D  \ts \t : \tau}
%\quad\quad
%\infer  {\G ; \D  \ts \unbx{\t} :  \tau}
%        {\G ; \D  \ts \t : \bxed{\tau}}
%$}} 

\hline 


%{Return}
\infer[\rlabel{return}]
{\G ; \D  \ts \ret{\t} : \tau}
{\G ; \emptyContext  \ts \t : \tau}
\\[4mm]

%{Let!}

\infer[\rlabel{let!}]
{ \G ; \D  \ts \letbin{x \cdcolon \eta}{\t}{\e} :\tau}
{ \G ; \D  \ts \t : \bang{\eta} &  \G, x \cc \eta; \D \ts \e : \tau}
\\[4mm]

% Split
%{Let$\cross$}
\infer[\rlabel{let$\cross$}]
        {\G ; \D \ts \letpin{a_1\cc\taui}{a_2\cc\tauii}{\t}{\e} :\tau}
        {\G ; \D  \ts \t :\taui \cross \tauii & 
         \G ; \D,a_1 \cc \taui,a_2 \cc \tauii \ts \e : \tau}
\\[4mm]


%{Case}
\infer[\rlabel{case}]
{\G ; \D \ts  \caseofflat{\t}{\ai}{\taui}{\ei}{\aii}{\tauii}{\eii} : \tau}
{
\begin{array}{rcl}
\G ; \D & \ts & t : \taui \osum \tauii \\
\G ; \D,\ai\cc\taui & \ts & \ei : \tau\\
\G; \D,\aii\cc\tauii & \ts & \eii : \tau
\end{array}
}
\end{array}
\]
}
\caption{Typing judgments for terms (top) and expressions.}
\label{fig:term-static}
\end{figure}

%% Exp typings
\begin{figure}[h]
\fixedCodeFrame{
\small
%\setlength{\tabcolsep}{0ex}
\[
\begin{array}{c}
%{Return}
\infer[\rlabel{return}]
{\G ; \D  \ts \ret{\t} : \tau}
{\G ; \emptyContext  \ts \t : \tau}
\\[4mm]

%{Let!}

\infer[\rlabel{let!}]
{ \G ; \D  \ts \letbin{x \cdcolon \eta}{\t}{\e} :\tau}
{ \G ; \D  \ts \t : \bang{\eta} &  \G, x \cc \eta; \D \ts \e : \tau}
\\[4mm]

% Split
%{Let$\cross$}
\infer[\rlabel{let$\cross$}]
        {\G ; \D \ts \letpin{a_1\cc\taui}{a_2\cc\tauii}{\t}{\e} :\tau}
        {\G ; \D  \ts \t :\taui \cross \tauii & 
         \G ; \D,a_1 \cc \taui,a_2 \cc \tauii \ts \e : \tau}
\\[4mm]


%{Case}
\infer[\rlabel{case}]
{\G ; \D \ts  \caseofflat{\t}{\ai}{\taui}{\ei}{\aii}{\tauii}{\eii} : \tau}
{
\begin{array}{rcl}
\G ; \D & \ts & t : \taui \osum \tauii \\
\G ; \D,\ai\cc\taui & \ts & \ei : \tau\\
\G; \D,\aii\cc\tauii & \ts & \eii : \tau
\end{array}
}
\end{array}
\]}

\caption{Typing judgments for expressions.}
\label{fig:expr-static}
\end{figure}

%\begin{figure}
%\fbox{\parbox{5in}{
%\begin{eqnarray*}
% \bang{\tau} & := & \Box \circ \tau\\
% \bang{\t} & := & \mbox{box}(\mbox{val} (\iota (\t)))\\
% \ret{\t} & := & \mbox{box}~(\iota (\t)) \\
% \letbin{x:\tau}{\t}{\e} & := &  
%  \mbox{let}~\Box~x : \tau ~\mbox{be}~\mbox{let}~\Box~y : \tau~\mbox{be}~t~
% \mbox{in}~ y~ \mbox{in}~ e
%\end{eqnarray*}
%}}
%\end{figure}

